SPINE: Online Semantic Planning for Missions with Incomplete Natural Language Specifications in Unstructured Environments

As robots become increasingly capable, users will want to describe high-level missions and have robots infer the relevant details. Because pre-built maps are difficult to obtain in many realistic settings, accomplishing such missions will require the robot to map and plan online. While many semantic planning methods operate online, they are typically designed for well specified missions such as object search or exploration. Recently, Large Language Models (LLMs) have demonstrated powerful contextual reasoning abilities over a range of robotic tasks described in natural language. However, existing LLM-enabled planners typically do not consider online planning or complex missions; rather, relevant subtasks and semantics are provided by a pre-built map or a user. We address these limitations via SPINE, an online planner for missions with incomplete mission specifications provided in natural language. The planner uses an LLM to reason about subtasks implied by the mission specification and then realizes these subtasks in a receding horizon framework. Tasks are automatically validated for safety and refined online with new map observations. We evaluate SPINE in simulation and real-world settings with missions that require multiple steps of semantic reasoning and exploration in cluttered outdoor environments of over 20,000m$^2$. Compared to baselines that use existing LLM-enabled planning approaches, our method is over twice as efficient in terms of time and distance, requires less user interactions, and does not require a full map. Additional resources are provided at https://zacravichandran.github.io/SPINE.

==> Makefile <==
# @fclad
# Simple makefile to compile paper with latexmk. Change DIR_OUTPUT for
# a tmpfs path, you really don't want to use your write cycles of your
# SSD compiling a paper

NAME = root
LATEX = latexmk -pdf -bibtex -pvc -jobname=$(NAME)
DIR_OUTPUT = /tmp/Volatile

## Sources
SRC = $(NAME).tex

.PHONY	: all clean \
          essay

all 	: essay

essay 	:
	$(LATEX) $(SRC) > /dev/null

# @fclad
# A better clean is rm -rf / but that may have unintended consequences
clean	:
	@-rm -f $(DIR_OUTPUT)/$(NAME)*

